Stratified Prediction-Powered Inference for Hybrid Language Model Evaluation

Prediction-powered inference (PPI) is a method that improves statistical estimates based on limited human-labeled data. PPI achieves this by combining small amounts of human-labeled data with larger amounts of data labeled by a reasonably accurate -- but potentially biased -- automatic system, in a way that results in tighter confidence intervals for certain parameters of interest (e.g., the mean performance of a language model). In this paper, we propose a method called Stratified Prediction-Powered Inference (StratPPI), in which we show that the basic PPI estimates can be considerably improved by employing simple data stratification strategies. Without making any assumptions on the underlying automatic labeling system or data distribution, we derive an algorithm for computing provably valid confidence intervals for population parameters (such as averages) that is based on stratified sampling. In particular, we show both theoretically and empirically that, with appropriate choices of stratification and sample allocation, our approach can provide substantially tighter confidence intervals than unstratified approaches. Specifically, StratPPI is expected to improve in cases where the performance of the autorater varies across different conditional distributions of the target data.

==> checklist.tex <==
\newpage
\section*{NeurIPS Paper Checklist}


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All claims are supported in the paper.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We address this in the conclusion.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Proofs are included in the appendix.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{}{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Results are based on publically available data, and simulations, and all procedures are described.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The data is publicly available, and the methodology is simple to implement. Pseudocode is given. Code may be made available at a future date.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Detailed information is provided.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Error bars are provided for the main experimental results.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Compute resources required are very light, as no model training is performed.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: No issues.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper discusses the advantages of the method for more effective development of large language models.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: NA
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: NA
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: NA
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: NA
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: NA
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}


\end{document}

==> sections/05a_partition_results.tex <==
\subsection{Continuous autorater predictions and stratified estimators}



%In the experiments above, we considered discrete-valued autoraters and human ratings.  This is an appropriate assumption in many cases (notably, when prompted LLM autoraters are used) but it is also common to use fine-tuned autorater models which output a calibrated probability.  

\newcommand{\bst}[1]{\textbf{#1}}
\newcommand{\ours}{\textit{ours:}}

\begin{table*}[tb]
\begin{center}
\begin{tabular}{lrrrr|rrrr}
\toprule
 &  \multicolumn{4}{c}{CI Width}
 & \multicolumn{4}{c}{CI Ratio to Classical} \\
 Method & Seahorse1 & Seahorse2 & AQA1 & AQA2 & Seahorse1 & Seahorse2 & AQA1 & AQA2 \\
\midrule
 & \multicolumn{8}{c}{\textit{methods that do not tune hyperparameters on $S_n$}} \\
\midrule
classical & 0.112 & 0.107 & 0.108 & 0.112  & 1.000 & 1.000 & 1.000 & 1.000\\
difference estimate & 0.098 & 0.104 & 0.099 & 0.096 & 0.873 & 0.968 & 0.914 & 0.855\\
\ours{} chain rule & 0.100 & 0.102 & 0.094 & 0.094  & 0.892 & 0.951 & 0.870 & 0.833 \\
\ours{} stratified($K=5$) 
& \bst{0.094} & \bst{0.100} & \bst{0.084} & \bst{0.080}  
& \bst{0.839} & \bst{0.929} & \bst{0.778} & \bst{0.708}  \\
\midrule
 & \multicolumn{8}{c}{\textit{methods that tune on $S_n$}} \\
\midrule
tree(5) & 0.093 & 0.100 & 0.082 & 0.079 & 0.829 & 0.932 & 0.765 & 0.703 \\
stratified($K=*$) & 0.092 & 0.099 & 0.082 & 0.079  & 0.826 & 0.919 & 0.759 & 0.701 \\
%\midrule
%& \multicolumn{8}{c}{\textit{adding powertuning}} \\
difference estimate + ptune  & 0.095 & 0.100 & 0.089 & 0.089 & 0.848 & 0.928 & 0.825 & 0.788\\
stratified($K=5$) + ptune  & 0.093 & 0.099 & 0.082 & 0.078 & 0.826 & 0.916 & 0.764 & 0.688 \\
stratified($K=*$) + ptune & 0.092 & 0.098 & 0.081 & 0.077 & 0.822 & 0.914 & 0.748 & 0.685 \\
tree($K=5)$ + ptune
& \bst{0.091} & \bst{0.097} & \bst{0.078} & \bst{0.075} 
& \bst{0.808} & \bst{0.902} & \bst{0.726} & \bst{0.668} \\
%tree($K=5$) + powertune & 0.090 & 0.097 & 0.079 & 0.075 & 0.800 & 0.893 & 0.732 & 0.664 \\
\bottomrule
\end{tabular}
\end{center}
\caption{CI widths and CI width ratio for all datasets with $n=300$ human-labeled examples.  Methods marked with ``+ ptune'' use powertuning \cite{angelopoulos2023ppi} within partitions. 
The difference estimate baseline is implemented as in \cite{doi:10.1126/science.adi6000}.  All methods that include tuning are novel (``ours'') except for the difference estimate with power tuning (called PPI++ in \cite{angelopoulos2023ppi}).}
\label{tab:n300}
\end{table*}

\begin{figure*}[t]
\begin{center}

\begin{tabular}{cc}
 \includegraphics[width=0.35\textwidth]{figures/seahorseq4.png} & 
 \includegraphics[width=0.35\textwidth]{figures/seahorseq5.png} \\
 \includegraphics[width=0.35\textwidth]{figures/aqa-rtr.png} & 
 \includegraphics[width=0.35\textwidth]{figures/aqa-posthoc.png} \\
\end{tabular}
\end{center}
\caption{Comparing stratified estimates on multiple datasets.  On all graphs, the $x$ axis is number of human-labeled examples $n$, and the $y$ axis is confidence interval width.  All PPI methods improve over classical approaches.  The chain rule estimate and difference estimate are generally comparable, and the stratified estimate improves performance substantially over each of them (see Section~\ref{sec:impact-part}).}
\label{fig:part}
\end{figure*}

\begin{table}[htb]
    \centering
    \begin{tabular}{lrrrr}
\toprule
 Method & SH1 & SH2 & AQA1 & AQA2 \\
 \midrule
 classic & 96.6 & 96.5	& 97.8	& 97.3 \\
 difference est & 96.9 &95.5 & 98.8	& 99.0 \\
 chain rule & 97.4 & 96.4 & 98.3	& 98.9 \\
 strat($K=5)$ & 96.3 & 95.8 & 97.3	& 97.0 \\
 \midrule
 tree($K=5$) & 96.3 & 95.7 & 96.3 & 95.5 \\
 tree($K=*$) & 92.2 &  88.5 & 91.3 & 89.4 \\
 strat($K=*$) & 96.9 & 95.7 & 97.6 & 96.9 \\
 \multicolumn{5}{l}{\textit{$+$ powertune}} \\
 difference est & 97.6 & 95.9 & 99.3 & 98.5 \\
 strat($K=*$) & 96.8 & 95.7 & 97.5 & 96.4 \\
 tree($K=5$ & 96.3 & 95.8 & 95.5 & 95.1 \\
 tree($K=*)$ & 89.7 & 87.7 & 87.7 & 86.1 \\
 \bottomrule
    \end{tabular}
    \caption{Coverage results at $n=300$ for 1000 trials of each method. All methods, even the tuned methods, obtained coverage at least as large as the expected 95\% except for those that combine regression-tree learning with search over the optimal number of partitions.}
    \label{tab:coverage-300}
\end{table}

\subsubsection{Datasets}

A common task in NLP is evaluating long-form outputs from LLMs: for instance, the outputs of chatbots, summarizers, and systems that provide long answers to information-seeking questions.  In general this is done with human ratings, and for many tasks, autoraters also exist.  In this setting, there will be a limited set of gold ratings $x,z,y$,
and two LLM models: a \emph{generator model} which produces answer an output $z$ from an input prompt $x$, and a \emph{autorater model} which takes a pair $x,z$ and outputs a predicted human rating $\hat{y}$.

As the first testbed for these tasks, we use data from the Seahorse project \cite{clark-etal-2023-seahorse}.  In this work, the authors considered generator models that summarize a source document $x$ in a multilingual setting.  This is a compelling task since obtaining labels for multiple languages is expensive.  Seahorse also includes labels for many languages, many systems, and many dimensions of summary quality: overall there are labels for 6 dimensions of summary quality, for 9 summarization systems, and 6 languages.  

We consider here two quality dimensions, one which captures if the summary is fully attributable to the source document, and one which captures if the summary captures the main idea of the source.  (These are the dimensions for which there was the greatest variance between different summarization models. )  We consider one summarization system---a finetuned 13B parameter multilingual mT5 \cite{xue2020mt5} model, the strongest model based on an open-source LLM.  The judge models for each dimension are also mT5-XXL finetuned models, which output probability scores.  The data contains 2728 examples for these two task, all of which have both human ratings and autoratings.  

As a second testbed we used data distributed by the authors of \cite{bohnet2023attributed}, which compared many models on the task of \emph{attributed question answering}.  In attributed question answering, the goal of the QA system is to output an answer and a document that supports that document---i.e., a generation $z$ is a pair $(a_x,d_x)$ where $a_x$ is an answer to question $x$, and $d_x$ is a document $d_x$ that supports the answer, and the generation is considered correct $(y=1)$ if the answer is indeed supported by the document.  We evaluated two ``generator'' models from \cite{bohnet2023attributed}: the highest-scoring ``retrieve-and-read'' QA system\footnote{RTR-10 in the dataset. Retrieve-and-read (RAG) models use a dense retriever with $x$ as query to find candidate documents $d_x$ from a corpus and then generate an answer $a_x$ with a fine-tuned LLM that takes $d_x$ as context.}, and the highest-scoring ``post-hoc retrieval'' system.\footnote{Post-6 in the dataset.  Post hoc retrieval systems generate an answer $a_x$ and then search for a supporting document $d_x$ using $a_x$ as a query.}  
The autorater for this task is a natural-language entailment model: a 11B parameter T5 \cite{JMLR:v21:20-074} model fine-tuned on a collection of NLI-related tasks \cite{honovich2022true}, which again gives probability scores.  These datasets have 1000 human labels and 3000 autorater labels.

\subsubsection{Initial experimental results}

Following \cite{doi:10.1126/science.adi6000} we evaluate PPI method performance using the \emph{width} of a confidence/credible interval. Using $\ell_e, u_e$ for the classical confidence interval for the estimand $e$ and $\ell_g,u_g$ for the PPI confidence interval of the designed statistic $g$, the \emph{width of the classical confidence interval} is $u_e - \ell_e$, and similarly for the PPI interval.  We also consider the \emph{CI width ratio}, which we define as $\frac{u_g - \ell_g}{u_e - \ell_e}$, i.e., the CI width of a PPI test normalized by the width of the classical test.

We compare the classical estimate, which uses only the human labels $S_n$ to a stratified model with $K=5$ equal-frequency partitions.  We did not tune the number of partitions at all in these initial experiments.  We also compare to the difference estimate (called simply PPI in the experiments of \cite{angelopoulos2023ppi,doi:10.1126/science.adi6000}), and, for completeness, the chain rule estimate.  The chain rule estimate is designed for discrete autoraters, and was used here by discretizing the autorater scores using a threshold of 0.5.    The difference estimate baseline is the classical method \cite{doi:10.1126/science.adi6000}, not the Bayesian version described Table~\ref{tab:methods}.

The top rows of Table~\ref{tab:n300} shows these results, averaged over 1000 trials each.

We also use the  experimental procedure of \cite{doi:10.1126/science.adi6000} to simulate the performance of statistical tests with varying numbers of human labels $n$.  We pick 10 different numbers $n$ ranging from 100 to 500, and for each value of $n$, we sample $n$ of the cases with human labels for the human-labeled set $S_n$, and use all the remaining autorater labels as $\twid{S}_N$.  We repeat this 100 times for each value of $n$, and graph the average CI width over all trials for 95\% confidence intervals.  These results are shown in Figure~\ref{fig:part}.

As shown in Table~\ref{tab:n300} at $n=300$, the difference estimate performs surprisingly well, and is comparable and to the chain rule estimate perform similarly on all dataset, despite not having access to the autorater's actual numeric scores.  As expected, the stratified estimate gives a noticeable improvement over the others. 

There is a larger improvement for all PPI methods in the attributed QA tasks: note that one important difference between the Seahorse data and the attributed QA data is that English-language entailment is a well-studied problem with large amounts of training data available, so one would expect the autorater here to be strong.  

Figure~\ref{fig:part} adds nuance to this view, showing that the stratified methods performs less well comparatively with small $n$, but improves over other methods substantially for larger $n$.  This makes sense, because there will be variance associated with the rectifier in each partition, and this variance will be larger when the partition has few human-labeled examples.  Additional experiments exploring this are in Appendix~\ref{app:seahorse}.  
The crossover between the stratified estimate with $K=5$ and the difference estimate is between $n=100$ and $n=150$ for these datasets.%---at which point there are 20-30 human-labeled examples in each partition.


\subsubsection{Practical implications} \label{sec:impact-part}

The graphs of Figure~\ref{fig:part} make it fairly easy to see the practical impact of the improved test.  As an example, drawing a horizontal line on the lower right-hand graph at around $y=0.10$ shows that similar confidence sized confidence intervals using 200 examples of the stratified estimate as using 400 examples of the classical estimate, so in this case labeling costs could be potentially reduced by half.  On the upper right-hand graph, where the differences between methods are smaller, a line in the same $y$ position shows that 300 examples with the stratified estimate are as useful as around 360 labels for the classical method, a 20\% reduction in labeling.

\subsubsection{Coverage tests}

%https://docs.google.com/spreadsheets/d/1kCpg7ezvEroGPRWeTSNpqAw50Jxn1JRFkn7wV-Pq6R4/edit?resourcekey=0-SO7NjpkAO04a-V2rakSxcQ#gid=0

The other important property for a statistical test to have, of course, is that an interval be calibrated: e.g., that a 95\% interval contain the true value of the parameter at least 95\% of the time.  Since for each of these tasks, a fairly large human-labeled dataset is available, we used the mean value obtained using all the human-labeled data as a proxy for the ``true'' value of the unknown parameter $\theta^*$, an measured test \emph{coverage}, i.e., how often the interval given by each test contains this $\theta^*$.  For a 95\% confidence interval, this should occur 95\% of the time.

In Figure~\ref{fig:part}, we aggregate all the tests for each method and each task, so there are a total of sixteen cases, with 1000 intervals considered for each case.  In each case the coverage was 95\% or greater, as expected, with the minimum coverage estimate being 95.5\% (for the difference estimate on the ``Main Points'' Seahorse dimension).
In conducting the experiments for Figure~\ref{fig:vary-part-k}, the stratified estimate was run 1000 times each for 4 values of $K$.  In each of the four cases the coverage was 97.2\% or greater, confirming the theoretical predictions.

% coverage https://docs.google.com/document/d/1TEPY08prWTGYTYsnBVD4TLwwuYRPbP3zsD3eqAEyBjM/edit?resourcekey=0-c7xpJHGMz_InpgApknVV2g&tab=t.0
% https://docs.google.com/spreadsheets/d/1kCpg7ezvEroGPRWeTSNpqAw50Jxn1JRFkn7wV-Pq6R4/edit?resourcekey=0-SO7NjpkAO04a-V2rakSxcQ#gid=0



\subsubsection{Tuning and powertuning PPI estimates} \label{sec:tuning}

In statistical testing, one must be wary of conducting multiple tests and choosing the best, as this can lead to results that are not well-calibrated---i.e., the true parameter value will lie outside the suggested confidence interval more frequently than expected.  This is why in the experiments of Figure~\ref{fig:part} we used a fixed $K=5$ for the number-of-partitions hyperparameter.   

In many practical settings, however, it is necessary to evaluate systems on many related tasks: e.g., one consider scaling the Seahorse data from 9 languages to 90, or evaluating dozens of variants of a chatbot system during development.  In such settings it is certainly plausible to tune a PPI estimate on a subset of the available tasks and run the well-tuned task on the others, eliminating any multiple-test worries.  Past experiments of \cite{angelopoulos2023ppi} also show that power tuned models seem to be well-calibrated even when the $\lambda^*$ parameter is set by (re-)using $S_n$.
(Recall from Section~\ref{sec:powertune-related} that \emph{powertuning} generalizes the difference method to
\[
 g(S_n, \twid{S}_N) 
   = \frac{1}{N}\sum_{j=1}^N \lambda f(x_j)
   ~~+~~ \frac{1}{n}\sum_{i=1}^n y_i - \lambda f(x_i)    
\]
for any $\lambda$ and also provides a method for picking a $\lambda*$ to minimize variance, thus finding the best test in a family.)

In summary, even if some gaps remain in our formal understanding of the practice of tuning PPI estimates with the labeled data, it seems important to consider these techniques.  In this section we consider methods for tuning hyperparameters of these methods.

\label{sec:reg-tree}

Tuning $K$ is conceptually easy---one can simply run the method with different values of $K$ and adopt the $K^*$ that gives the smallest variance. More generally, the way in which partitions are constructed could also be varied, by intelligently picking partitions to be as large as possible subject to the constraint that $y-\hat{y}$ stays roughly constant within partitions.  One easy-to-implement version of this idea is to fit a regression tree \cite{lewis2000introduction} to the labeled data, using the autorater score $\hat{y}$ as an input feature and the human label $y$ as the target value, and then use the leaves of the tree as partitions.

The bottom rows of Table~\ref{tab:n300} presents results for a variety of tuned PPI methods.  We first present the regression-tree partitioning method, constrained to output a tree with at most $K=5$ leaves, and varying the number of partitions $K$ for the equal-frequency partitions with and without powertuning (see Appendix~\ref{app:seahorse} for details.).  We then consider adding powertuning to all methods (except the chain rule.)  Many of these methods lead to substantially improved results, with the powertuned regression-tree method performing best.




\subsubsection{Coverage Tests}

Without a strong theory that predicts coverage for tuned PPI methods, experiments on coverage are essential. 
The results for each result in Table~\ref{tab:n300} are averaged over 1000 trials each, and we recorded for each of these trials the coverage of the method (i.e., how often the CI contains the true value, as estimated from all available human-labeled examples.)  The results are shown in Table~\ref{tab:coverage-300}.  Interestingly, all of the methods, including those that use tuning, are still well-calibrated, \emph{except} for the ones that combine tree learning and search over $K$ (shown as ``tree($K=*$)'' in the table.)  The poor coverage results for these methods are why their CI widths are not presented in Table~\ref{tab:n300}.

==> sections/05b_chain_results.tex <==
\subsection{Uncalibrated autoraters and chain-rule estimates} \label{sec:openqa}

The previous section considers autoraters that are based on well-calibrated, fine-tuned models.  A common recent practice is to use prompted models for autoraters, which we consider next.  Note that some of the strategies available for fine-tuned models cannot be used here: in particular, since only a few different predictions are made by autoraters, partitioning cannot be used effectively.

\subsubsection{Datasets}

In a recent paper \cite{kamalloo-etal-2023-evaluating} showed that the most commonly-used metrics for evaluating open-book QA systems are very biased, relative to human raters.  Among other results, they evaluated 10 widely-used open-book QA systems on 3600 examples with automatically-computed metrics, such as exact-match or token-F1 similarity to known answers, and also evaluated the same systems with human raters on a smaller set of 300 examples.  The human ratings are very different (see Table~\ref{tab:kamalloo-motivate}), showing gains in accuracy of more than 20\% in several cases.
The authors discuss potential solutions, including using prompted LLMs as autoraters, but ultimately conclude ``At this time, there appears to be no substitute for human evaluation [of open-book QA systems].''

\begin{table}
\centering
\begin{tabular}{l|rr|rr}
\toprule
     & EM & F1 & Human & (delta) \\
     & \multicolumn{2}{c}{3.6k examples} & \multicolumn{2}{|c}{300 examples} \\
\midrule
DPR &  40.9 & 47.8 & 58.8 & +12.9 \\
FiD & 46.5 & 53.7 & 64.8 & +17.0 \\
ANCE/FiD & 47.3 & 54.8 & 65.8 & +17.6 \\
RocketQAv2/FiD  & 47.7 & 55.6 &  70.1 & +20.3 \\
Contriever/FiD  & 47.9 & 55.4 & 66.5 & +20.0 \\
FiD-KD  & 49.6 & 57.4 &  73.1 & +22.3 \\
GAR+/FiD & 49.8 & 57.4 & 69.4 & +18.2 \\
EviGen  & 49.8 & 57.0 & 67.1 & +15.3 \\
EMDR2  & 51.5 & 59.5 &  73.1 & +19.9 \\
R2-D2  & 52.4 & 59.0 &  71.4 & +18.6 \\
\bottomrule
\end{tabular}
\caption{Human vs automatic labels for open-book QA systems, from \cite{kamalloo-etal-2023-evaluating}.}
\label{tab:kamalloo-motivate}
\end{table}

We experimented with the data released by \cite{kamalloo-etal-2023-evaluating}. The data includes model outputs for ten models on 3600 examples, but only includes human labels for the smaller set of 300 examples.  Since PPI methods require a larger set of autorater examples, we implemented an prompted autorater using Gemini Pro \cite{team2023gemini}, and ran this autorater on the the question/answer pairs for every model on each of the 3.6K standard NQ test examples, resulting in 300 human labels and 3.3k autorater labels for each model.  Similar to the autoraters of \cite{kamalloo-etal-2023-evaluating}, our autorater takes a question/answer pair, plus the set of known short answers, and predicts if the answer is acceptable or not.  No probability scores are associated with an autorating.

We elected to evaluate performance at $n=300$ labeled examples exclusively, rather than constructing curves as in Figure~\ref{fig:part}.

\subsubsection{An abstaining, uncalibrated autorater} \label{sec:abstain}

Our model is prompted to produce binary values, but occasionally outputs results that are cannot be easily parsed into a correct/incorrect decision.  A principled way of dealing with this was discussed in Section~\ref{sec:abstain-method}: we use the chain rule estimater, and model the LLM as producing an ``unknown'' value as a third possible outcome for the random variable $A$, which now could take on the values ``y'' (for an acceptable question/answer pair), ``n'' (for an unacceptable pair), or ``u'' for an uncertain result. 

%This dataset offers one kind of uncertain result---an unparsable response from the autorater.  This is a quite common outcome for LLM autoraters.
%Of course, this same method could be used to estimate confidence for an autorater that has been designed to answer ``unknown'' for cases that are hard to determine, but we leave that for future work.

\begin{figure}[t]
\begin{center}
    \includegraphics[width=0.45\textwidth]{figures/kamalloo-ci-overview.png}
\end{center}
\caption{Confidence intervals for the chain rule  estimate with abstentions, the difference estimate, and the classical method for the open-book QA methods from \cite{kamalloo-etal-2023-evaluating}.} \label{fig:kamaloo-cis}
\end{figure}

\begin{table}[t]
\centering
\begin{tabular}{lcl}
\toprule
            & mean interval & width ratio\\
            & width         & to classical\\
\midrule
classical   & 0.105 & 1.00 \\
difference estimate & 0.096 & 0.92\\
chain rule estimate & 0.089 & 0.85 \\
\bottomrule
\end{tabular}
\caption{Summary of confidence interval sizes at $n=300$ with an abstaining autorater for the data of \cite{kamalloo-etal-2023-evaluating}, averaged over 10 models.  Applying the difference estimate requires linearizing the autorater scores (see text).} \label{tab:kamalloo-summary-abstain}
\end{table}

\begin{table}[t]
\centering
\begin{tabular}{lcl}
\toprule
            & mean interval & width ratio\\
            & width         & to classical\\
\midrule
classical   & 0.105 & 1.00 \\
difference estimate & 0.095 & 0.91\\
chain rule estimate & 0.085 & 0.81\\
\midrule
 & \multicolumn{2}{c}{\textit{tuning on $S_n$}} \\
\midrule
difference est + ptune & 0.083 & 0.79 \\
\bottomrule
\end{tabular}
\caption{Summary of confidence interval sizes with a binary autorater for the data of \cite{kamalloo-etal-2023-evaluating}, averaged over 10 models.  The autorater was engineered to ``back off'' to exact match when the prompted model abstained (see text) } \label{tab:kamalloo-summary}
\end{table}

As summarized in Figure~\ref{fig:kamaloo-cis} and 
Table~\ref{tab:kamalloo-summary-abstain} confidence intervals produced by the chain rule estimate are about 15\% smaller than the classical intervals, and about 8\% smaller than the difference estimate intervals. \footnote{Notice that to use the difference estimate, it is necessary to map the unordered discrete values ``n'', ``y'', and ``u'' into real numbers: we made the natural assignment of $n=0$, $y=1$, and $u=0.5$, which makes the values similar to the binary 0/1 values used for the human rating.  Other options are discussed in Appendix~\ref{sec:linear}.}

For this dataset, there is another reasonable strategy for handling unparseable judge model responses, namely, ``backing off'' to the exact-match evaluation metric which is traditionally used for evaluation of open-book answers. Doing this improves both the chain rule estimate and the difference estimate slightly (as shown in the top Table~\ref{tab:kamalloo-summary}, but the chain rule still performs best.

If we consider tuned methods, we note that adding powertuning to the difference estimate improves performance significantly for these tasks. As shown in the bottom section of Table~\ref{tab:kamalloo-summary}, the power-tuned difference estimate slightly outperforms the chain rule estimate.

\subsubsection{Practical implications}

Although a 20\% reduction in width may seem modest, because confidence shrink with the square root of the number of labeled data, the number of labels needed may be reduced dramatically due to a small reduction in CI width.  Showing curves like those of Figure~\ref{fig:part} for all ten models is impractical, so
following \cite{doi:10.1126/science.adi6000} we subsampled the available human-labeled data to find the smallest sample size $n_\textit{min}$ that would give a confidence interval the same width or smaller than the baseline interval obtained by running the classical method on all available data.  The results, shown in Table~\ref{tab:kamalloo-min-n}, indicate that only 60\% of the data need be labeled to get estimates that are just as precise.  (These results use the best untuned model above, i.e., the chain rule estimate with backoff instead of abstentions.) 

We also estimated the number of examples $n^+$ that would need to be human-labeled to get the chain-rule estimate's interval width using the classical method.  The average $n^+$ for these tasks is 465, or about 57\% more labels (not shown in any table or figure).

\begin{table}
\centering
\begin{tabular}{llcc}
\toprule
{} &                 &  $n_\textit{min}$  with &  $n$ with \\
 &                    & chain rule & classical\\
 &                    & interval & interval \\
\midrule
 &             DPR &    151 &          291 \\
 &             FiD &    129 &          300 \\
 &   ANCE/FiD &    137 &          300 \\
 &    RocketQAv2/FiD &    185 &          299 \\
 &  Contriever/FiD &    141 &          300 \\
 &          FiD-KD &    150 &          300 \\
 &    GAR/FiD &    151 &          300 \\
 &          EviGen &    155 &          299 \\
 &           EMDR2 &    241 &          274 \\
 &            R2-D2 &    175 &          300 \\
 \midrule
 & average & 161.5 & 296.3 \\ 
\bottomrule
\end{tabular}
\caption{Minimal number of human-labeled examples $n_\textit{min}$ for the chain rule to obtain a confidence interval width smaller than the classical interval width using all available human-labeled examples. } \label{tab:kamalloo-min-n}
\end{table}

\subsubsection{Coverage tests} \label{sec:coverage}

Without large human-labeled sets, it is not possible to determine if the confidence intervals produced include the true values of $\theta^*$.  We thus used synthetic data 
to conduct coverage tests: for details, see Appendix~\ref{sec:kamaloo-coverage}.  Again we experimented with the best untuned model above. 

On 1000 synthetic datasets, the ``true'' $\theta^*_H$ used to generate the data was included in the 95\% confidence interval all but 48 times, or 95.2\% of the time. 

%\wc{repeat tests with PPI++}

% individual runs: [40, 48, 46, 45, 48, 42, 48, 38, 51, 51, 50, 38, 52, 54, 42, 37, 43, 40, 42, 43]


%\wc{update - and do this in frequentist setting?}
%Repeating an appropriate variant of the coverage tests of Section~\ref{sec:coverage}, we find the true $\theta^*_H$ included in the confidence interval all but 51 times in 1000 trials, or 5.1\% of the time, showing this model is also well-calibrated.


==> sections/05c_sxs_results.tex <==

\subsection{Designing a PPI method for side-by-side tests} \label{sec:sxs-results}

One claimed advantage of the Bayesian approach is that it is straightforward to design a new PPI method.
We now consider constructed such a new method for side-by-side tests---to our knowledge, no PPI method for this task exists.

In side-by-side tests, raters (human $H$ or automatic $A$) label a pair $x$ with $w$, $l$, or $t$, for win, loss, or tie.  In the example of evaluating of question-answering systems, $x$ would contain a question and two answers (one from a baseline method, and one from a proposed improvement) and $f(x)$ predicts the human response with $\hat{y} \in \{w,l,t\}$. As before we assume a small set $S_n$ with both human and autorater labels and a larger dataset $\twid{S}_N$ with only autorater labels.

The goal of side-by-side tests is to see if the proposed method outperforms the baseline.  We formalize this with a statistic that tests to see if wins are more likely than losses:
\[ e(S_n, \twid{S}_N) \equiv \hat{\mu}_{Hw} - \hat{\mu}_{Hl}
\]
where
\begin{eqnarray*}
    \hat{\mu}_{Hw} & = & \prop{H=w}{S_n} \\
   \hat{\mu}_{Hl} & = & \prop{H=l}{S_n}   
\end{eqnarray*}
The designed statistic is a straightforward extension of the chain rule estimate.  We use the chain run to define autorater-assisted versions of $\hat{\mu}_{Hw}$ and $\hat{\mu}_{Hl}$ and then subtract them.
\begin{small}
\begin{eqnarray*}
   \hat{p}_{A=a} & = & \prop{A=a}{\twid{S}_N} ~,~ \mbox{for~} a\in\{w,l,t\} \\
   \hat{p}_{H=w|a} & = & \cprop{H=w}{A=a}{\twid{S}_N} ~,~ a\in\{w,l,t\} \\
   \hat{p}_{H=l|a} & = & \cprop{H=l}{A=a}{\twid{S}_N} ~,~  a\in\{w,l,t\} \\
    %q_{H=w} & \stackrel{\scriptsize{\rm def}}{\equiv} & \sum_{a \in \{w,l,t\}} \hat{p}_{H=w|a} \cdot \hat{p}_{A=a} \\
    %q_{H=l} & \stackrel{\scriptsize{\rm def}}{\equiv} & \sum_{a \in \{w,l,t\}} \hat{p}_{H=l|a} \cdot \hat{p}_{A=a} \\
 g(S_n,\twid{S}_N) & = &  \sum_{a \in \{w,l,t\}} \hat{p}_{H=w|a} \cdot \hat{p}_{A=a} ~ -  ~ \hat{p}_{H=l|a} \cdot \hat{p}_{A=a} 
\end{eqnarray*}
\end{small}


\subsubsection{Data and experimental procedure}

Freely available, high quality side-by-side labeled data for pairs of models is difficult to obtain.  However, when the same outputs of two different have been individually labeled, it is easy to simulate side-by-side ratings: e.g., if model $A$'s output on input $x$ is rated as ``good'' and model $B$'s output on $x$ is rated as ``bad'',  then one can rate $x$ as a ``win'' for $A$.  The same process can be used to simulate an autorater that produces side-by-side ratings.  Hence for for simulated side-by-tests, we used again the attributed QA data distributed by the authors of \cite{bohnet2023attributed}.

We began by finding a set of pairs of models $M_1, M_2$ such that (1) both models are competitive (2) neither model makes use of the autorater internally and (3) $M_1$ outperforms $M_2$.  We then used a multiple hypothesis test to find a set of 59 pairs $M_1, M_2$ where every $M_1$ outperforms $M_2$ with 95\% confidence (using a classical paired test on proportions and all the human data).  

We then reran the classical test and the method of Sec~\ref{sec:sxs} with subsamples of various sizes, ranging from 50 to 1000, as in the experiments above, and averaged over ten trials.

\subsubsection{Results and practical implications}

The results are shown in Figure~\ref{fig:pairs}.  The $x$ axis is the number of human-labeled examples used, and the $y$ axis is the fraction of the 59 pairs that can be separated at a 95\% confidence level.  We only compared the chain-rule test and a classical paired test, as previously published PPI tests are not directly applicable to paired tests,
and our prior experiments in linearizing discrete scores for difference estimates suggest that doing this effectively requires substantial exploration (see Appendix~\ref{tab:linearize}.)

As the figure shows, the chain rule test is dramatically different according to this measure: for example, with 100 examples, only 54\% of the pairs were separable with the classical test, verses 76\% with the chain rule test, and with 200 examples, the corresponding numbers are 79\% and 94\%.

\begin{figure}[t]
\begin{center}
    \includegraphics[width=0.45\textwidth]{figures/pairs.png}
\end{center}
\caption{Fraction of pairs of truly different systems that can be distinguished by a paired test, with classical methods and a chain rule estimate.} \label{fig:pairs}
\end{figure}

\subsubsection{Coverage tests}  \label{sec:aqa-coverage}

We ran synthetic-data experiments similar to those of Section~\ref{sec:coverage} for the side-by-side estimates, as detailed in Appendix~\ref{sec:kamaloo-coverage}.  On 1000 synthetic datasets, the ``true'' $\theta^*_H$ used to generate the data was included in the 95\% confidence interval 94.5\% of the time, which is not statistically significant lower than the expected result ($p$-value of 0.46 using a classical test.)

==> sections/05d_freq_results.tex <==
\subsection{Non-Bayesian experimental results}

To clarify the claims of this paper, we do not suggest that the methods here improve on prior methods simply because they are Bayesian.  Rather, we claim that (1) for PPI, Bayesian approaches are analytically simpler, facilitating development of new PPI methods which are (2) experimentally preferable to prior PPI methods.

\subsubsection{Discussion}

Let us begin this section with a short discussion of Bayesian {\it vs.} frequentist approaches to confidence intervals.  Recall a Bayesian \emph{credible interval} for parameter $\theta$, for \emph{confidence level} $c$, is a pair of values $\ell$ and $u$ such that 
\[
    \int_{\ell}^u f(\theta) d\theta = c
\]
where $f(\theta)$ as the posterior of a random variable $\theta$ given data $D$, $f(\theta)=p(\theta|D)$.  In this framework, the interval $\ell, u$ for level $c$ means that $p(\ell \leq \theta \leq u) \geq c$, where the probability is taken over the possible values of the unknown parameter $\theta$.

In a classical (frequentist) confidence interval, the same relationship between $f$, $\ell$, and $u$, and $c$ holds, but $f(\theta)$ is not a posterior of anything---it's just a pdf, depending on the data $D$, that has been designed to satisfy the constraint above.  To be precise about the classical claim, let us use $\theta*$ for the unknown and fixed parameter value,
and write $f=f_S$ to show its dependence on $S$.  A frequentist construction for $f$ is correct if
\begin{equation} \label{eq:freq}
    \forall \theta*, \ell, u: 
 p_{S}(\ell \leq \theta* \leq  u) = 
   \int_\ell^u f_{S}(\theta) d\theta
\end{equation} 
where $p_S$ means that the probability is taken over samples drawn according to $\theta*$, i.e., $S \sim p(S|{\theta*})$.

To compare these two interpretations briefly, the Bayesian approaches require a posterior over $\theta$, which in turn requires a prior. This is a double-edged sword: you can inject subjective knowledge about $\theta$ easily if you have it, but you have to make up some sort of prior even when you don't.  However, credible intervals are easy to compute for many cases (as we see above).   In contrast, the classical interpretation requires (and allows) no prior on $\theta$, but is a bit harder to make sense of, and in our experience it is often confused with the Bayesian credible-interval interpretation (especially by ML researchers who have been exposed to Bayesian methods).  It's also technically difficult to establish that a method satisfies Eq~\ref{eq:freq}, although of course classical tests for most common situations exist.

We emphasize, however, that while there is definitely a \emph{conceptual} difference between treating the sample $S$ as a random variable (in the classical setting) and treating the parameter $\theta$ as a random variable (in the Bayesian setting), the practical differences are less dramatic.  Usually there is only one $\theta$ and one $S$, and unsurprisingly the computations for classical and Bayesian  work out to be quite similar: in each case, one picks a pdf $f(\theta)$ and snips off the tails.  For the case of means, the two pdfs are identical.  For the case of proportions, fitting a Beta with a Jeffrey's prior to a sample produces generally produces curves almost identical to the Gaussians used in the Wald method.\footnote{The exception is for small $n$ and extreme $\theta$, where an exact test would be preferred, and here the Beta closely approximates the binomial of Clopper-Pearson test.}

\subsubsection{Experimental results}

The discussion above suggests that the Bayesian credible intervals explored here might also perform well according to frequentist goals.  To evaluate this, we re-visited the coverage experiments of Section~\ref{sec:coverage}, where 1000 synthetic datasets were produced with different (but plausible) ``true'' parameters $\theta^*$.  As expected, about 5\% of these led to coverage failures---i.e., the chain-rule confidence interval did \emph{not} contain $\theta^*$.  In a Bayesian setting, this sort of failure is fine, since the probability for the interval is taken over different values of $\theta^*$; however, the frequentist interpretation of confidence intervals requires a 95\% interval contain the true value of the parameter for \emph{every} true value, where the probability is taken over samples---i.e., synthetically generated datasets.  

To evaluate performance according to the frequentist goal, we returned to the experiments of Section~\ref{sec:coverage},  randomly selected 20 of the $\theta*$'s which led to coverage failures in the initial set of 1000 trials, and re-generating 1000 synthetic datasets for each of these problematic $\theta^*$'s.
The fraction of coverage failures on this set of 20,000 simulations was 4.49\% overall.  Considering the 20 values for $\theta*$ separately, each of the 1000 $\theta*$-specific runs had between 37 and 54 coverage failures, showing the technique is well-calibrated in a frequentist sense as well.  We performed a similar\footnote{To reduce cost, here we ran a total of 1000 trials, where in each trial we selected one random coverage-failing $\theta^*$ from the 55 observed, and regenerated a dataset from that.} experiment with the data from Section~\ref{sec:aqa-coverage} and obtained similar results, with an overall coverage-failure rate of 3.9\%.

\subsubsection{The bootstrap as alternative to Monte Carlo integration}

Our approach also relies on Monte Carlo integration, a Bayesian approach.
An alternative to using Monte Carlo integration to evaluate CIs for proxy estimands is the bootstrap \cite{wasserman2013all}, which makes no explicit Bayesian assumptions.

The bootstrap can be used to compute expected values and confidence intervals over any numeric function $g(S)$ computed on a sample $S$.  In bootstrapping, one creates  $B$ \emph{bootstrap replicates}
$S^1, \ldots, S^B$ and then computes $g^1=g(S^1), \ldots, g^B=g(S^B)$.  A bootstrap replicate is simply a dataset of size $|S|$ that is formed by randomly sampling $|S|$ elements of $S$ with replacement.  The results of applying $g$ to each replicate are handled same way as the results of applying $g$ to samples from the posterior in Monte Carlo integration.  (In fact, our use of Monte Carlo integration is closely related to \emph{parametric bootstrapping} \cite{efron2012bayesian}.)

Compared to Monte Carlo integration, bootstrapping is slower, since samples of $g$ require time $O(N)$, instead of constant time.  However, bootstrapping does not require parameter independence, and does not require picking priors for each parameter.  Although the arguments behind the correctness of bootstrap are
different, it behaves similarly on these tasks.  For instance, we repeated the experiments of Table~\ref{tab:kamalloo-summary} using bootstrapping instead of Monte Carlo integration, and results that were numerically almost identical: e.g., the chain rule estimate's average width was measured as 0.084358 with the bootstrap, and 0.084516 with Monte Carlo integration.



==> sections/cuts.tex <==
As an example, the difference estimate can be defined as
\begin{eqnarray*}
\hat{\mu}^{N}_{f(x)} & = & \mean{f(x)}{x}{\twid{S}_N} \\
\hat{\mu}^{n}_{y-f(x)} & = & \mean{y - f(x)}{(x,y)}{S_n} \\
g(S_n, \twid{S}_N) & = & \hat{\mu}^{N}_{f(x)} + \hat{\mu}^{n}_{y-f(x)}
\end{eqnarray*}

In general, we will assume there is a statistic, the \emph{target estimand}, we want to measure in expectation.  For the difference estimate this is
\[  e(S_n,\twid{S}_N, f) \equiv \mean{y}{(x,y)}{S_n}
\]
In each method described below, we will introduce a second statistic, the \emph{proxy estimand}, that has the same expectation as $g$ but lower variance. For the difference estimate the proxy estimand is
\[  g(S_n,\twid{S}_N, f) \equiv  \hat{\mu}_{f(x)} + \hat{\mu}_{y-f(x)}
\]
We must verify analytically that $\expect{g}=\expect{e}$, but will measure variance experimentally.  This is easy to do, since confidence intervals on $g$ can be computed automatically using Monte Carlo integration. (For details and an example of doing this, see Appendix~\ref{sec:python}.) 


-----




PPI is useful and quite general, being based on theories of convex optimization, but it can be difficult to map specific use-cases into PPI. Here we advocate for methods that require only designing a \textit{statistic} which is a function of several \textit{estimates}, and then computing confidence intervals over this statistic.  For the task of Figure~\ref{fig:h100-vs-ar-5000}, we would like to design a statistic that equals $p(H)$ in expectation, but which has a tighter confidence interval.

Bootstrap:

Assume a statistic $g(S_n)$ computed on a sample $S$.

Given sample $S$, create $B$ \emph{bootstrap replicates}
$S^1, \ldots, S^B$ and then compute $g'^1=g(S^1), \ldots, g'^B=g(S^B)$.
Sort these low to high to form a vector $\overline{g'}$, which is an empirical sample of $g(S'|S_n)$.  Given $\alpha$, the lower limit $\ell_g$ of a confidence interval for $1-\alpha$ is found by dropping the lowest $B \alpha/2$ elements of $\overline{g'}$ and taking the lowest remaining value as $\ell_g$,  and the upper limit by dropping the highest $B \alpha/2$ elements and taking the highest remaining value.

\wc{robustness/guarantees}

\wc{relative cost, robustness}

\wc{for Monte Carlo integration}

-----

The \emph{difference estimator} is discussed in more detail below in Sec~\ref{sec:diff-est}: briefly, it is a way of obtaining a tighter confidence interval for an estimate of the mean of some value $y$, if one is given access to a small sample with true values of $y$
and a larger sample of approximate values of $y$.

----



----



We can thus estimate $p(AR=1)$ accurately since we can run the autorater on large sample (above, $n=5000$).  Also note that if the autorater is good, then $p(H=1|AR=1)$ should be close to one, and $(1-p)$ is small and we can also estimate this well, and likewise $p(H=1|AR=0)$ should be close to zero and also can be estimated well.  For this task, we thus use the three estimates
\begin{eqnarray*} 
\hat\theta_{AR=1}  & \mbox{estimated from 5000 auto-rated examples} \\
\hat\theta_{H=1|AR=1} & \mbox{estimated from 100 dual-labeled examples} \\
\hat\theta_{H=1|AR=0} & \mbox{estimated from 100 dual-labeled examples} \\
\end{eqnarray*}
Letting $\boldsymbol{\theta}$ denote $\langle \hat\theta_{AR=1}, \hat\theta_{H=1|AR=1}, \hat\theta_{H=1|AR=0} \rangle$ 
we define the statistic $s(\boldsymbol{\theta})$ as
\[
s(\boldsymbol{\theta}) \equiv
    \hat\theta_{H=1|AR=1} \cdot \hat\theta_{AR=1} + 
    \hat\theta_{H=1|AR=0} \cdot (1 - \hat\theta_{AR=1})
\]
Since $s(\boldsymbol{\theta})$ is just a definition of $p(H=1)$ using the chain rule and $p(AR)$, it is an unbiased estimator for $p(H=1)$, but for strong autorater AR, $s$ will have a small confidence interval.  

What remains is the question of how to \emph{compute} a confidence interval for $s(\boldsymbol{\theta})$, of more generally any statistic based on estimates.
Below we describe below two methods doing this. One is based on the bootstrap, a frequentist non-parametric approach, and one is based on \emph{parametric bootstrap}, which also has a Bayesian justification.

Our hope is that simple approaches to designing and implementing auto-rater assisted statistical tests will unlock novel approaches to making use of autoraters for evaluation in statistically justified ways.  To support this, we present a series of case studies showing how autorater-assisted statistical tests can be designed and empirically verified.
